Matching Tasks to Objectives: Fine-Tuning and Prompt-Tuning Strategies for Encoder-Decoder Pre-trained Language Models

Prompt-based learning has emerged as a dominant paradigm in natural language processing. This study explores the impact of diverse pre-training objectives on the performance of encoder-decoder pre-trained language models across generation and question answering tasks, with a focus on commonsense knowledge retrieval and completion. We highlight the benefits of incorporating multiple objectives during both pre-training and fine-tuning stages. We introduce the Match Task to Objective (MTO) framework and methods for determining the appropriate objective for a given task. This framework offers automated methods to prepare task-related data for adaptation through unsupervised training, based on the identified objective. In the fine-tuning stage, we design novel templates that align with the objectives of the pre-training and adaptation stages. When aligned with task requirements, these strategies can achieve a performance gain of over 120\% compared to conventional methods in few-shot settings. They significantly outperform related works in few-shot settings and exceed the baseline even in full-dataset scenarios. Furthermore, we extend this approach to include prompt-tuning methodologies, providing guidance for more effective soft prompt engineering and optimization. Our strategies significantly enhance prompt-tuning performance as well. These insights hold substantial value, precisely guiding the selection and optimization of models customized for specific tasks. Code is available at https://github.com/puraminy/MTO/

==> ff.tex <==
%\documentclass{article}
%\usepackage{makecell}
%\usepackage{booktabs}
%\usepackage{caption}

%\begin{document}		
	\begin{table*}[h!]
		\centering
		\begin{tabular}{lcccccc}
			\toprule
			\textbf{Methods} & \multicolumn{3}{c}{\textbf{CommonSenseQA}} & \multicolumn{3}{c}{\textbf{OpenBookQA}} \\
			\cmidrule(lr){2-4} \cmidrule(lr){5-7}
			& \makecell{FS \\ 30} & \makecell{5\% \\ 425} & \makecell{20\% \\ 1700} & \makecell{FS \\ 30} & \makecell{5\% \\ 298} & \makecell{20\% \\ 991} \\
			\midrule
			RoBERTa-large     & -- & 29.66 & 58.47 & -- & 37.00 & 41.47 \\
			MHGRN           & -- & 29.01 & 50.23 & -- & 38.00 & 39.73 \\
			QA-GNN          & -- & 32.95 & 50.15 & -- & 33.53 & 42.40 \\
			GreaseLM        & -- & 22.80$^\star$ & 63.09$^\star$ & -- & 39.00$^\star$ & 42.20$^\star$ \\
			GSC \cite{base-GSC}            & -- & 31.02$^\star$ & 65.83$^\star$ & -- & 29.60$^\star$ & 42.40$^\star$ \\
			SAFE            & -- & 36.45 & 65.16 & -- & 38.80 & 44.93 \\
			MVP-Tuning      & -- & 48.99 & 67.12 & -- & 39.60 & 56.00 \\					         
			\midrule
			\multicolumn{7}{c}{Our Methods (Fine-Tuning)} \\
			\midrule   
			T5-large (baseline)        & 21.04 & 23.12 & 65.15 & 23.34 & 43.08 & 55.31 \\      
			T5-MP           & 25.11 & 25.53 & 59.02 & 21.26 & \textbf{54.42} & $\mathbf{57.52}^d$ \\  
			T5-MAP          & $\textbf{48.21}_c^d$ &  $60.05^{d}$ & \textbf{68.12} & $35.84_c$ & 40.24 & $44.3^{l}$ \\ 
			T5-AP           & $ 47.01^l$ & \textbf{$\mathbf{61.22}^d$} & $66.25^d$ & \textbf{39.71} & 46.72 & 48.63 \\  
			\midrule
			\multicolumn{7}{c}{Our Methods (Prompt-Tuning)} \\
			\midrule
			T5-PreMAP          & $35.28^d$ & $ \underline{52.35}^d$ & $ \underline{59.21}^l$ & $22.63^l$ & $34.33^l$ & $ 33.15^l $ \\  
			T5-PreAP          & $19.14^d$ & $33.41^l$ & $59.17$ & $3.15^d$ & $32.71^l$ & $33.27^l$ \\  
			\bottomrule
		\end{tabular}
		\caption{Comperison of proposed method with related works on CommonSenseQA and OpenBookQA datasets.}
	\end{table*}
	
%\end{document}


==> ft-bscore.tex <==
\begin{tabular}{llllllllll}
\hline
 lm           & unsup        & unsup-nat  & \textbf{0.47} & \textbf{0.50} & 0.45          & 0.41          & 0.47          & \textbf{0.47} & \textbf{0.53} \\
 base         & sup          & unsup-nat  & \textbf{0.47} & \textbf{0.50} & \textbf{0.46} & 0.43          & 0.47          & 0.41          & \textbf{0.53} \\
 v1           & unsup        & unsup-nat  & \textbf{0.47} & 0.48          & \textbf{0.46} & \textbf{0.44} & \textbf{0.50} & 0.46          & 0.52          \\
\hline
\end{tabular}

==> ft-cs-mis.tex <==

	\begin{table}[htbp]
		\centering
		\begin{tabular}{|c|c|c|}
			\toprule
			\textbf{Model} & \textbf{Version} & \textbf{Accuracy} \\
			\midrule
			\multirow{4}{*}{base}  & MaskedChoicePrompting & 94.25 \\
			& MaskedAnswerPrompting & 88.84 \\
			& AnswerPrompting & 95.48 \\
			& ChoicePrompting & 94.62 \\
			\midrule
			\multirow{4}{*}{large} & MaskedChoicePrompting & 95.31 \\
			& MaskedAnswerPrompting & 94.19 \\
			& AnswerPrompting & 98.61 \\
			& ChoicePrompting & 99.39 \\
			\bottomrule
		\end{tabular}
		\caption{Model version accuracy comparison}
		\label{table:accuracy}
	\end{table}



==> hscore.tex <==
\begin{tabular}{llllllllll}
\hline
 model   & objective   & template   & Avg.           & \rot{AtLocation}    & \rot{CapableOf}     & \rot{HasProperty}   & \rot{ObjectUse}     & \rot{isFilledBy}    & \rot{xAttr}         \\
\midrule
\multicolumn{10}{c}{\textbf{Rouge Scores}} \\
\midrule
 t5-lm           & Denoising        & MP  & \textbf{0.18} & 0.16          & 0.19          & 0.13          & 0.21          & \textbf{0.21} & \textbf{0.18} \\
 t5-base         & LM          & MP  & \textbf{0.18} & \textbf{0.20} & \textbf{0.20} & \textbf{0.18} & 0.20          & 0.12          & \textbf{0.18} \\
 t5-v1           & Denoising        & MP  & \textbf{0.18} & 0.16          & 0.19          & 0.17          & \textbf{0.22} & 0.19          & 0.14          \\
\midrule
\multicolumn{10}{c}{\textbf{Bert Scores}} \\
\midrule
t5-lm           & Denoising        & MP  & \textbf{0.47} & \textbf{0.50} & 0.45          & 0.41          & 0.47          & \textbf{0.47} & \textbf{0.53} \\
t5-base         & LM          & MP  & \textbf{0.47} & \textbf{0.50} & \textbf{0.46} & 0.43          & 0.47          & 0.41          & \textbf{0.53} \\
t5-v1           & Denoising        & MP  & \textbf{0.47} & 0.48          & \textbf{0.46} & \textbf{0.44} & \textbf{0.50} & 0.46          & 0.52          \\
\hline
\end{tabular}

==> qatemps.tex <==
%\documentclass{article}
%\usepackage[table]{xcolor}
%\usepackage{multirow}
%\usepackage{xcolor}
%\usepackage{makecell}
%\usepackage{booktabs} % for \midrule

%\begin{document}
	
	\begin{table*}[th!]
		\centering
		\begin{tabular}{l | l | l}
			\toprule
			\multicolumn{3}{c}{\textbf{QA Fine-Tuning}} \\
			\midrule
			\multirow{1}{*}{\textbf{Template}} &  \\
			& \textit{Input} & \textit{Target} \\
			\hline         		
			AnswerPrompting & \makecell{Choice1: Oven Choice2: Refrigerator \\  Where do you put food to keep it cold?} & \makecell[l]{Refrigerator} \\
			\hline         		
			MaskedAnswerPrompting & \makecell{AnswerPrompting + \textcolor{brown}{\textbf{X}}} & \makecell[l]{\textcolor{brown}{\textbf{X}} Refrigerator} \\ 	
			\hline         		
			AnswerPromptingCH & \makecell{AnswerPrompting \\ + \textcolor{cyan}{the correct choice is}} & \makecell[l]{Choice2 Refrigerator} \\
			\hline         		
			MaskedAnswerPromptingCH & \makecell{MaskedAnswerPrompting \\ + \textcolor{cyan}{the correct choice is} \textcolor{blue}{\textbf{Y}}} & \makecell[l]{\textcolor{brown}{\textbf{X}} Refrigerator \\ \textcolor{blue}{\textbf{Y}} Choice2} \\
			\midrule
            \multicolumn{3}{c}{\textbf{QA Prompt-Tuning}} \\
            \midrule			
			PreAnswerPT & \makecell{\textcolor{red}{ $ \mathbf{P}_1 \mathbf{ P}_2  \dots  \mathbf{P}_n $} + AnswerPrompting} & \makecell[l]{Refrigerator} \\
			\hline
			PostAnswerPT & \makecell{AnswerPrompting + \textcolor{red}{ $ \mathbf{P}_1 \mathbf{ P}_2  \dots  \mathbf{P}_n $}} & \makecell[l]{Refrigerator} \\
			\hline
			PreMaskedAnswerPT & \makecell{\textcolor{red}{ $ \mathbf{P}_1 \mathbf{ P}_2  \dots  \mathbf{P}_n $} + MaskedAnswerPrompting} & \makecell[l]{\textcolor{brown}{\textbf{X}} Refrigerator} \\
			\hline
			PostMaskedAnswerPT & \makecell{MaskedAnswerPrompting + \textcolor{red}{ $ \mathbf{P}_1 \mathbf{ P}_2  \dots  \mathbf{P}_n $}} & \makecell[l]{\textcolor{brown}{\textbf{X}} Refrigerator} \\
			\hline
		\end{tabular}
		\caption{Templates for Formatting the Input and Output of an Encoder-Decoder Model during Fine-Tuning and Prompt-Tuning for Knowledge Completion and Question Answering Tasks.}
		\label{table:methods}
	\end{table*}
	
%\end{document}


==> results.tex <==
\begin{table*}[h!]
	\centering
	\begin{tabular}{lc|cc|c|cc}
		\toprule
		\textbf{Methods} & \multicolumn{3}{c}{\textbf{CommonSenseQA}} & \multicolumn{3}{c}{\textbf{OpenBookQA}} \\
		\cmidrule(lr){2-4} \cmidrule(lr){5-7}
		& \makecell{FS \\ 30} & \makecell{5\% \\ 425} & \makecell{20\% \\ 1700} & \makecell{FS \\ 30} & \makecell{5\% \\ 298} & \makecell{20\% \\ 991} \\
		\midrule
		RoBERTa-large     & -- & 29.66 & 58.47 & -- & 37.00 & 41.47 \\
		MHGRN           & -- & 29.01 & 50.23 & -- & 38.00 & 39.73 \\
		QA-GNN          & -- & 32.95 & 50.15 & -- & 33.53 & 42.40 \\
		GreaseLM        & -- & 22.80$^\star$ & 63.09$^\star$ & -- & 39.00$^\star$ & 42.20$^\star$ \\
		GSC \cite{base-GSC}            & -- & 31.02$^\star$ & 65.83$^\star$ & -- & 29.60$^\star$ & 42.40$^\star$ \\
		SAFE            & -- & 36.45 & 65.16 & -- & 38.80 & 44.93 \\
		MVP-Tuning      & -- & 48.99 & 67.12 & -- & 39.60 & 56.00 \\					         
		\midrule
		\multicolumn{7}{c}{Our Methods (Fine-Tuning)} \\
		\midrule   
		T5-large        & 23.94 & 23.12 & 65.15 & 23.73 & 43.08 & 55.31 \\      
		MTO-MP           & 20.09 & 25.53 & 59.02 & 23.93 & \textbf{54.42} & $\mathbf{57.52}^d$ \\  
		MTO-MAP          & $\textbf{52.5}_c^m$ &  $60.05^{d}$ & \textbf{68.12} & $\textbf{38.47}^l_c$ & 40.24 & $44.3^{l}$ \\ 
		MTO-AP           & $ 49.28^m$ & \textbf{$\mathbf{61.22}^d$} & $66.25^d$ & 32.73 & 46.72 & 48.63 \\  
		\midrule
		\multicolumn{7}{c}{Our Methods (Prompt-Tuning)} \\
		\midrule
		MTO-PreMAP          & $35.28^d$ & $ \underline{52.35}^d$ & $ \underline{59.21}^l$ & $22.63^l$ & $34.33^l$ & $ 33.15^l $ \\  
		MTO-PreAP          & $19.14^d$ & $33.41^l$ & $59.17$ & $3.15^d$ & $32.71^l$ & $33.27^l$ \\  
		\bottomrule
	\end{tabular}
	\caption{Comparison of the proposed method with related works on CommonSenseQA and OpenBookQA datasets.}
	\label{results-qa}
\end{table*}


==> stat.tex <==
\begin{table}[h]
	\centering
	\begin{tabular}{llcc}
		\toprule
		\textbf{Dataset} & \textbf{Split} & \textbf{Average Question Length (words)} & \textbf{Average Choice Length (words)} \\
		\midrule
		commonsense\_qa & Train & 13.25 & 1.52 \\
		openbookqa & Train & 10.71 & 2.78 \\
		commonsense\_qa & Test & 13.43 & 1.51 \\
		openbookqa & Test & 10.30 & 3.06 \\
		\bottomrule
	\end{tabular}
	\caption{Statistics for Commonsense QA and Openbook QA datasets}
	\label{tab:qa_stats}
\end{table}

==> tables/large-filling.tex <==
\begin{tabular}{rllllllllll}
\hline
   model & objective   & template      & AtLocation    & CapableOf     & HasProperty   & ObjectUse     & isFilledBy    & xAttr         & All           & metric                  \\
\hline
\hline
     nan & LM          & MP            & \textbf{0.53} & 0.48          & 0.39          & \textbf{0.53} & 0.45          & 0.52          & \textbf{0.48} & \multirow{5}{*}{BERT}   \\
     nan & LM          & Prompting     & 0.50          & \textbf{0.50} & 0.40          & 0.50          & \textbf{0.47} & \textbf{0.53} & \textbf{0.48} &                         \\
     nan & LM          & Mapping       & 0.47          & 0.47          & \textbf{0.41} & 0.50          & 0.45          & 0.52          & 0.47          &                         \\
     nan & ---         & Mapping       & 0.45          & 0.39          & 0.38          & 0.42          & 0.46          & 0.52          & 0.44          &                         \\
     nan & LM          & MaskedMapping & 0.47          & 0.45          & 0.40          & 0.47          & \textbf{0.47} & 0.50          & 0.46          &                         \\
\hline
     nan & LM          & MP            & \textbf{0.23} & 0.23          & 0.13          & \textbf{0.25} & 0.16          & 0.11          & 0.18          & \multirow{5}{*}{Rouge}  \\
     nan & LM          & Prompting     & 0.22          & \textbf{0.24} & 0.16          & 0.23          & \textbf{0.19} & 0.13          & \textbf{0.19} &                         \\
     nan & LM          & Mapping       & 0.15          & 0.21          & \textbf{0.19} & 0.20          & 0.17          & 0.10          & 0.17          &                         \\
     nan & ---         & Mapping       & 0.10          & 0.08          & 0.02          & 0.04          & 0.16          & \textbf{0.14} & 0.09          &                         \\
     nan & LM          & MaskedMapping & 0.17          & 0.18          & 0.10          & 0.18          & \textbf{0.19} & 0.11          & 0.16          &                         \\
\hline
\end{tabular}

==> tables/large-map.tex <==
\begin{tabular}{rlllllll}
\hline
   model & objective   & template   & xIntent       & xNeed         & xWant         & All           & metric                  \\
\hline
\hline
     T5-large & LM          & Mapping    & \textbf{0.57} & \textbf{0.57} & \textbf{0.55} & \textbf{0.56} & \multirow{1}{*}{BERT}   \\
\hline
     T5-large & LM          & Mapping    & \textbf{0.48} & \textbf{0.43} & \textbf{0.38} & \textbf{0.43} & \multirow{1}{*}{Rouge}  \\
\hline
\end{tabular}

==> tables/pt-base.tex <==
\begin{tabular}{lllllllllll}
\hline
 model   & objective   & template     & AtLocation    & CapableOf     & HasProperty   & ObjectUse     & isFilledBy    & xAttr         & All           & metric                  \\
\hline
\hline
 T5-base & Mixed       & MaskedPostPT & \textbf{0.52} & \textbf{0.41} & \textbf{0.38} & \textbf{0.45} & \textbf{0.44} & \textbf{0.49} & \textbf{0.45} & \multirow{0}{*}{BERT}   \\
\hline
 T5-base & Mixed       & MaskedPostPT & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \multirow{0}{*}{BLEURT} \\
\hline
 T5-base & Mixed       & MaskedPostPT & \textbf{0.20} & \textbf{0.13} & \textbf{0.13} & \textbf{0.16} & \textbf{0.20} & \textbf{0.14} & \textbf{0.16} & \multirow{0}{*}{Rouge}  \\
\hline
\end{tabular}

==> tables/results-kb-pt-top.tex <==
\begin{tabular}{rrrlllll}
\hline
   model &   objective &   template & xIntent        & xNeed          & xWant          & All            & metric                  \\
\hline
\hline
     nan &         nan &        nan & \textbf{56.43} & \textbf{53.75} & \textbf{51.22} & \textbf{53.80} & \multirow{0}{*}{BERT}   \\
\hline
     nan &         nan &        nan & nan            & nan            & nan            & nan            & \multirow{0}{*}{BLEURT} \\
\hline
     nan &         nan &        nan & \textbf{46.99} & \textbf{39.69} & \textbf{39.26} & \textbf{41.98} & \multirow{0}{*}{Rouge}  \\
\hline
\end{tabular}

==> tables/top-ft-map.tex <==
\begin{tabular}{llllllll}
\hline
 AtLocation    & CapableOf     & HasProperty   & ObjectUse     & isFilledBy    & xAttr         & All           & metric                       \\
\hline
\hline
 \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \multirow{2}{*}{bert-score}  \\
 \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} &                              \\
\hline
 nan           & nan           & nan           & nan           & nan           & nan           & nan           & \multirow{2}{*}{bleu-score}  \\
 nan           & nan           & nan           & nan           & nan           & nan           & nan           &                              \\
\hline
 0.05          & 0.13          & 0.02          & 0.12          & 0.04          & 0.04          & 0.07          & \multirow{2}{*}{rouge-score} \\
 \textbf{0.16} & \textbf{0.15} & \textbf{0.18} & \textbf{0.20} & \textbf{0.19} & \textbf{0.20} & \textbf{0.18} &                              \\
\hline
\end{tabular}

==> tables/tt.tex <==
\begin{tabular}{lllll}
\hline
 xIntent       & xNeed         & xWant         & All           & metric                       \\
\hline
\hline
 0.20          & 0.27          & \textbf{0.28} & 0.25          & \multirow{2}{*}{rouge-score} \\
 \textbf{0.44} & \textbf{0.41} & 0.20          & \textbf{0.35} &                              \\
\hline
 0.13          & \textbf{0.25} & \textbf{0.21} & \textbf{0.20} & \multirow{2}{*}{rouge-score} \\
 \textbf{0.17} & 0.20          & 0.11          & 0.16          &                              \\
\hline
 0.00          & 0.12          & \textbf{0.10} & 0.07          & \multirow{2}{*}{rouge-score} \\
 \textbf{0.46} & \textbf{0.32} & 0.03          & \textbf{0.27} &                              \\
\hline
\end{tabular}

==> top-ft-map.tex <==
\begin{tabular}{lllllll}
\hline
 model-base   & model-temp   & template   & All           & xIntent       & xNeed         & xWant         \\
\hline
 v1           & sup          & sup-nat    & \textbf{0.38} & 0.40          & \textbf{0.39} & 0.34          \\
 base         & unsup        & unsup-nat  & 0.37          & \textbf{0.41} & 0.38          & 0.33          \\
 lm           & unsup        & sup        & 0.37          & 0.39          & 0.37          & \textbf{0.35} \\
\hline
\end{tabular}

==> tt.tex <==
\begin{tabular}{lllll}
\hline
 xIntent       & xNeed         & xWant         & All           & metric      \\
\hline
 0.20          & 0.27          & \textbf{0.28} & 0.25          & bert-score  \\
 \textbf{0.44} & \textbf{0.41} & 0.20          & \textbf{0.35} & bert-score  \\
 \hline
 0.13          & \textbf{0.25} & \textbf{0.21} & \textbf{0.20} & bleu-score  \\
 \textbf{0.17} & 0.20          & 0.11          & 0.16          & bleu-score  \\
 \hline
 0.00          & 0.12          & \textbf{0.10} & 0.07          & rouge-score \\
 \textbf{0.46} & \textbf{0.32} & 0.03          & \textbf{0.27} & rouge-score \\
\hline
\end{tabular}
